ASRJam: Human-Friendly AI Speech Jamming to Prevent Automated Phone Scams

Large Language Models (LLMs), combined with Text-to-Speech (TTS) and Automatic Speech Recognition (ASR), are increasingly used to automate voice phishing (vishing) scams. These systems are scalable and convincing, posing a significant security threat. We identify the ASR transcription step as the most vulnerable link in the scam pipeline and introduce ASRJam, a proactive defence framework that injects adversarial perturbations into the victim's audio to disrupt the attacker's ASR. This breaks the scam's feedback loop without affecting human callers, who can still understand the conversation. While prior adversarial audio techniques are often unpleasant and impractical for real-time use, we also propose EchoGuard, a novel jammer that leverages natural distortions, such as reverberation and echo, that are disruptive to ASR but tolerable to humans. To evaluate EchoGuard's effectiveness and usability, we conducted a 39-person user study comparing it with three state-of-the-art attacks. Results show that EchoGuard achieved the highest overall utility, offering the best combination of ASR disruption and human listening experience.

==> graveyard.tex <==
% \begin{itemize}
% \item \textbf{Proactive Defence: }
% We observe that the ASR component is the weakest link in the attacker's setup. If the defender can jam the ASR's functionality then the system fails. An innocent victim can activate ASR jamming in the call and know right away if she is conversing with an AI agent simply because the conversation no longer tracks (see Fig. \ref{fig:Attack_Defense_Framework}). ASR jamming is implemented by adding crafted noise, also known as an adversarial perturbation, to the target audio\cite{goodfellow2014explaining, carlini2018audio, alzantot2018did, neekhara2019universal}.This perturbation prevents the ASR from accurately transcribing what has been said. While white-box algorithms for creating perturbations exist \cite{carlini2018audio, lu2021exploring}, the defender in this case is limited to the use of zero-query black-box attacks (such as \cite{abdullah2021hear, ge2023advddos}). Here, 'black-box' implies the attack operates without knowledge of the target model's internal architecture or parameters, and 'zero-query' means the defender cannot probe the attacker's ASR with numerous queries to optimize the perturbation.

% \item \textbf{Practical ASR Jamming.:} The problem with existing jamming attacks is that the pertubation, while effective at corrupting ASR models, is very unpleasant for humans to hear during a phone call. Since the proposed defense must jam all \textbf{suspicious} calls, there is a possibility that legitimate callers (humans) will have to listen to the jamming noise while conversing with the defended individual. This is a critial issue for the proposed defense since if the defense is unpleasant to legitimate callers, then the defence is not usable (impractical). Therefore, we propose a new ASR jamming algorithm called \textbf{ASRJam} which not only black box, universal, effiecenit for real time applicaitons, but also more pleasent to listen to during a phone call than other STOA jammers. It accomplishes this by leveraging naturally occuring sound distortions that the human brain is well devleoped to process but ASR models are not due to various limitatiosn such as trainign bias. For example, echos are common since the time of caves... but an ASR model (especially pretrained) is not balanced towards echoes.  
% \end{itemize}




% First we suggest the idea of using offensive security: 


% we suggest targeting the weakest link of the pipeline which is the STT component. By adding adversarial noise, we can it is already known that there are ways to jam TTS systems using noise [][][] or   using a well known attack (1)  defence system which employs ASR jamming...
% % One wa

% Our research addresses this critical threat by targeting the STT component of the vishing pipeline. We hypothesize that there exists an audio transformation capable of significantly disrupting ASR models' transcription accuracy while having negligible impact on human intelligibility. By introducing transformations that exploit fundamental differences between human auditory systems and ASR models, we aim to prevent LLM-based scam systems from maintaining coherent and convincing conversations. These transformations are real-time, zero-query, and model-agnostic, ensuring their practicality and universality across diverse scenarios. Moreover, they are designed to introduce minimal interference in benign interactions, preserving the natural flow of human communication.
%  For an illustration of the danger and defense framework please see Figure~\ref{fig:Attack_Defense_Framework}


% This approach differs from traditional methods in the field of adversarial audio, which typically rely on perturbations designed to fool ASR models. While adversarial audio has made significant strides in demonstrating vulnerabilities in speech recognition, these methods often prioritize technical effectiveness at the expense of practical usability. Many approaches require prior knowledge of the target model, rely on repeated queries for optimization, or produce distortions that degrade human comprehensibility. These limitations make them unsuitable for real-time applications or settings where maintaining the naturalness of human communication is essential.


% Another relevant method is \textbf{Kenansville} \cite{abdullah2021hear}, which uses a surrogate model to craft universal perturbations transferable to unseen systems. It applies signal decomposition techniques such as Discrete Fourier Transform (DFT) and Singular Spectrum Analysis (SSA) to remove low-energy components before reconstruction. While effective, its reliance on surrogate models introduces practical limitations for purely zero-query setups.




% \section{Related Works}
% \label{sec:related_works}
% % adversarial attacks against audio have a rich history.... studied in whitebox [][][][] and many blackbox [][][][]. Both targeted and untargeted as well.  However in this work we are primarily focused on adversarial attacks that are universal, blackbox, zero query. Therefore we consider a few highly relevant attacks...


% Machine Learning (ML) models, particularly deep learning architectures, have achieved remarkable performance in tasks such as image classification \cite{krizhevsky2012imagenet, szegedy2015going, he2016deep}. However, these models are vulnerable to adversarial attacks—intentional, subtle perturbations to input data that cause models to produce incorrect outputs. Early research in adversarial machine learning focused on image classification models, demonstrating that imperceptible changes to images could lead to misclassification \cite{goodfellow2014explaining, szegedy2013intriguing}. For instance, \cite{kurakin2016adversarial} showed that adding minimal perturbations to images could deceive classifiers, while \cite{carlini2017towards} developed optimization-based attacks to bypass defensive distillation techniques.

% The concept of adversarial examples has extended to speech recognition systems, where audio inputs that sound benign to human listeners can cause models to produce incorrect or unexpected transcriptions. \cite{carlini2018audio} demonstrated that small perturbations to audio waveforms could force automatic speech recognition (ASR) systems to transcribe any desired text.

% Adversarial attacks can be categorized based on their objectives:

% \textbf{Targeted Adversarial Attacks.}
% These attacks aim to manipulate a machine learning model's output to a specific, adversary-chosen target. In the context of Automatic Speech Recognition (ASR) systems, this involves introducing subtle perturbations to audio inputs so that the system transcribes a predetermined phrase chosen by the attacker, regardless of the original content \cite{wu2023kenku, lu2021exploring, liu2024difattack}. For example, \cite{carlini2018audio} demonstrated that by adding minimal perturbations to audio samples, attackers could force ASR models to transcribe any desired text. This method leverages optimization techniques to craft perturbations that are inaudible to humans but cause targeted misclassification in ASR models.

% Similarly, \cite{yuan2018commandersong} introduced the "CommanderSong" attack, embedding malicious voice commands into songs. These commands are imperceptible to human listeners but are recognized by ASR models, highlighting the potential for stealthy command injection attacks.


% \textbf{Untargeted Adversarial Attacks.}
% In contrast to targeted methods, untargeted adversarial attacks aim to cause a machine learning model to produce any incorrect output, without specifying what that incorrect output should be. In the ASR domain, this means introducing perturbations that lead to incorrect transcriptions, thereby degrading the system's performance without directing it toward a specific erroneous phrase. For instance, \cite{alzantot2018did} proposed an untargeted attack using a genetic algorithm to find perturbations that lead to transcription errors.


% \subsection{Universal Adversarial Perturbations}

% Universal adversarial perturbations (UAPs) are input-agnostic noises that, when added to any audio sample, can mislead ASR models. \cite{neekhara2019universal} demonstrated the existence of UAPs capable of causing mis-transcriptions across various audio inputs when added to speech signals. Their algorithm crafted a single quasi-imperceptible perturbation that could fool ASR models like Mozilla DeepSpeech. However, the transferability of these perturbations to other models was limited, and human comprehensibility was not extensively evaluated.

% Building upon this, \cite{lu2021exploring} explored targeted UAPs for end-to-end ASR models, aiming to induce specific mis-transcriptions. Their findings indicated varying vulnerabilities among models, with some robustness observed against such perturbations. Nonetheless, the requirement for white-box access and potential perceptibility of perturbations limited practical applicability.

% \subsection{Zero-Query Adversarial Attacks}

% Zero-query adversarial attacks are particularly advantageous for real-time applications, as they do not require any access to the target model during the attack phase. These methods rely on pre-crafted perturbations that can generalize well across different models and inputs \cite{liu2024difattack}. Such approaches are essential in scenarios where querying the model is impractical or impossible, such as defending against LLM-based scammers.

% \cite{ge2023advddos} presented AdvDDoS, a zero-query adversarial attack on commercial speech recognition systems. This method utilized universal perturbations crafted without querying the target model, demonstrating high transferability. However, the study lacked a user evaluation to confirm the human comprehensibility of the adversarial examples.

% Another notable method, known as "Kenansville," employs a surrogate model to craft adversarial examples that deceive various target models without direct queries. This approach utilizes Discrete Fourier Transform (DFT) or Singular Spectrum Analysis (SSA) to decompose the input signal, discarding components below a certain threshold before reconstruction \cite{abdullah2021hear}.


% \subsection{Our Research Contributions}

% Existing adversarial attack methods on Automatic Speech Recognition (ASR) systems often lack one or more of the following essential attributes: universality, zero-query applicability, real-time execution, and human comprehensibility.

% \textbf{Universality and Real-Time Applicability:} Many attacks are not universal, requiring optimization for each input, which hinders real-time application. For instance, Liu et al. introduced a zero-query attack that necessitates per-input optimization, making it impractical for dynamic, real-time scenarios \cite{liu2024difattack}.


% \textbf{Zero-Query Applicability:} Numerous methods depend on querying the target model to generate effective adversarial examples. This reliance is problematic when the specific ASR model used by adversaries is unknown, rendering querying infeasible.

% \textbf{Human Comprehensibility:} Several studies lack thorough evaluation of how adversarial perturbations affect human perception. For example, AdvDDoS primarily uses the Signal-to-Noise Ratio (SNR) metric to assess noise levels, which may not accurately reflect human perceptual quality.

% Our research addresses these gaps by proposing a solution that is universal, zero-query, real-time applicable, and ensures human comprehensibility. This comprehensive approach offers a practical and effective defense mechanism against automated scams leveraging ASR models.



==> images/mainflow.tex <==
% \section{Diagrammatic view of Multisketch operations}\label{app:mainflow}  

% A user registers with a user id $\u$ and a vector of biometric templates
% $\mvec=\mvecss{\mlen}$. Multisketch uses two databases $\dbid$ and $\dbmsg$\@,
% where $\dbid$ contains user id $\u$ and the corresponding helper data
% $\sketchval$, and $\dbmsg$ contains the random permutation of the templates
% registered so far. Highlighted are the entries corresponding to a user $\u_4$
% with templates $\mvec_4=\mvec_{41}\ldots\mvec_{4\mlen}$.% and helper
%     % data $\sketchval_4$.
\begin{figure}[t]
  \centering
  \begin{tikzpicture}[
    >=stealth,
    node distance=2cm,
    database/.style={
      cylinder,
      cylinder uses custom fill,
      cylinder body fill=black!25!white,
      cylinder end fill=black!25!white,
      shape border rotate=90,
      aspect=0.25,
      minimum width=2em,
      minimum height=2em,
      draw
    },
    func/.style={
      rectangle,
      fill=red!25!white,
      minimum width=1cm,
      minimum height=1em,
      draw
    },
    cell/.style={
      rectangle,
      draw=black!50!white
    }
    ]
    \node (user) at (0, 0) {User};
    \node[func, right of=user, right=-1.1em, above=3em] (msketch) {$\MS$}; 
    \draw[below of=msketch, dashed, anchor=west] (.85,0.55) rectangle (5.9,-1.2); 
    \node[func, below of=msketch, anchor=east, below=1.95cm,fill=red!10!white,dashed] (mrecover) {$\MRec$};
    % \node[database, right of=user, anchor=south, above=1em, right=2cm] (db1) {$\dbid$};
    \matrix (db1) [right of=user, anchor=south, below=2pt, right=-0.1cm, 
    matrix of math nodes,
    column sep = -\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}}, 
    column 2/.style={nodes={cell}}, 
    anchor=west] {
      \u_1 & \sketchval_1\\
      \u_2 & \sketchval_2\\
      \u_3 & \sketchval_3\\
      |[draw,fill=blue!20]|\u_4 & |[draw,fill=blue!20]|\sketchval_4\\
    };
    \node[left of=db1, anchor=east,right=1.1cm] {$\dbid$};
    \matrix (db2) [right of=db1, left=25pt, matrix of math nodes,
    column sep = 2\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}},
    column 2/.style={nodes={cell}}, 
    column 3/.style={nodes={cell}}, 
    column 4/.style={nodes={cell}}, 
    column 5/.style={nodes={cell}}, 
    anchor=west] {
      \mvec_{21} &\mvec_{12} & |[draw,fill=blue!20]|\mvec_{43} &  & \mvec_{3\mlen} \\
      |[draw,fill=blue!20]|\mvec_{41} &\mvec_{32} & \mvec_{33} & |[draw=white]|\ldots & \mvec_{2\mlen} \\
      \mvec_{11} &|[draw,fill=blue!20]|\mvec_{42} & \mvec_{23} &  & \mvec_{1\mlen} \\
      \mvec_{31} &\mvec_{22} & \mvec_{13} & & |[draw,fill=blue!20]|\mvec_{4\mlen} \\
    };
    \node[left of=db2, left=-4pt] {$\dbmsg$};

    % \node[database,right of=db1] (db2) {$\dbmsg$};
    \node[func,below of=db1,anchor=north,above=8pt,left=8pt] (gu) {GetUser};
    \node[func,right of=gu,anchor=east,right=-5pt] (fm) {FindMatches};
    \node[func,below of=db1,anchor=east,below=2em,right=-3pt] (recover) {Recover};

    \draw[->,blue!50,thick] (user.north) |- node[black,near end,above]{$u, \mvec$} node[black,near end,below,font=\small]{register} 
    (msketch.west);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$u, \sketchval$} (db1);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$\mvec$} (db2);

    \draw[->,blue!50,thick] (user.south) |- ++(1,-0.9) node[black,near end,above]{$u, \mvectilde$} node[black,near end,below,font=\small]{login}   -| node[black,left,near end]{$u$}
    (gu.north);
    \draw[->,blue!50,thick] (user.south) |- ++(0,-0.9)  -- ++(3.1,0) |- node[black,near end, above]{$\mvectilde$}
    (fm.west);
    \draw[->,blue!50,thick] (db1.south) |- node[black,near end,above]{} (gu.east);
    \draw[->,blue!50,thick] (db2.south) |- node[black,near end,above]{} (fm.east);
    \draw[->,blue!50,thick] (gu.south) |- node[black,near end,above]{$\sketchval$} (recover.west);
    \draw[->,blue!50,thick] (fm.south) |- node[black,near end,above]{$\mvec'$} (recover.east);    
    \draw[->,blue!50,line width=2pt] (recover.south) -- node[black,near end,right]{$\mvec$ or $\bot$} ++(0, -0.65);
  \end{tikzpicture}
  % \rcnote{Rough sketch of the flow of the \biosketch.} 
  \caption{Diagram of multisketch as a part of an authentication service. 
  }
  \label{fig:mainflow}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> tables/librispeech_results.tex <==
\begin{table*}[htbp]
\centering
\caption{Attack Success Rate on \textbf{LibriSpeech} (\textuparrow = higher is better)}
\label{tab:librispeech_results}
\begin{tabular}{lcccccccc}
\toprule
\textbf{Method} & DS & W2V & Vosk & Whisper & SB & \cellcolor{gray!10}\textit{IBM} & \cellcolor{gray!10}\textit{MSFT} & \cellcolor{gray!10}\textit{Assembly} \\
\midrule
Kenku & 0.6696 & 0.1236 & 0.2999 & 0.0604 & 0.1025 & \cellcolor{gray!10}\textit{0.4748} & \cellcolor{gray!10}\textit{0.0200} & \cellcolor{gray!10}\textit{\textbf{0.0044}} \\
Kenansville & 0.2326 & 0.0470 & 0.1719 & 0.0522 & 0.0241 & \cellcolor{gray!10}\textit{0.3130} & \cellcolor{gray!10}\textit{0.0200} & \cellcolor{gray!10}\textit{\textbf{0.0044}} \\
AdvDDoS & 0.8578 & 0.1322 & 0.2907 & 0.0867 & \textbf{0.2130} & \cellcolor{gray!10}\textit{0.4611} & \cellcolor{gray!10}\textit{0.0222} & \cellcolor{gray!10}\textit{0.0100} \\
Ours & \textbf{0.9670} & \textbf{0.1489} & \textbf{0.4752} & \textbf{0.1419} & 0.0893 & \cellcolor{gray!10}\textit{\textbf{0.6333}} & \cellcolor{gray!10}\textit{\textbf{0.0252}} & \cellcolor{gray!10}\textit{0.0093} \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/spgi_results.tex <==
\begin{table*}[htbp]
\centering
\caption{Attack Success Rate on \textbf{SPGISpeech} (\textuparrow = higher is better)}
\label{tab:spgi_results}
\begin{tabular}{lcccccccc}
\toprule
\textbf{Method} & DS & W2V & Vosk & Whisper & SB & \cellcolor{gray!10}\textit{IBM} & \cellcolor{gray!10}\textit{MSFT} & \cellcolor{gray!10}\textit{Assembly} \\
\midrule
Kenku & 0.9342 & 0.7227 & 0.5815 & 0.1350 & \textbf{0.6756} & \cellcolor{gray!10}\textit{0.6955} & \cellcolor{gray!10}\textit{\textbf{0.0226}} & \cellcolor{gray!10}\textit{\textbf{0.0046}} \\
Kenansville & 0.7508 & 0.4054 & 0.4486 & 0.0447 & 0.3157 & \cellcolor{gray!10}\textit{0.6688} & \cellcolor{gray!10}\textit{0.0213} & \cellcolor{gray!10}\textit{0.0010} \\
AdvDDoS & 0.9721 & 0.5600 & 0.4113 & 0.0953 & 0.6659 & \cellcolor{gray!10}\textit{0.4305} & \cellcolor{gray!10}\textit{0.0128} & \cellcolor{gray!10}\textit{0.0005} \\
Ours & \textbf{0.9918} & \textbf{0.8311} & \textbf{0.7639} & \textbf{0.1636} & 0.5965 & \cellcolor{gray!10}\textit{\textbf{0.7125}} & \cellcolor{gray!10}\textit{0.0195} & \cellcolor{gray!10}\textit{0.0010} \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/tedlium_results.tex <==

\begin{table*}[htbp]
\centering
\caption{Attack Success Rate on \textbf{Tedlium} (\textuparrow = higher is better)}
\label{tab:tedlium_results}
\begin{tabular}{lcccccccc}
\toprule
\textbf{Method} & DS & W2V & Vosk & Whisper & SB & \cellcolor{gray!10}\textit{IBM} & \cellcolor{gray!10}\textit{MSFT} & \cellcolor{gray!10}\textit{Assembly} \\
\midrule
Kenku & 0.7446 & 0.3004 & 0.2070 & 0.0383 & 0.2410 & \cellcolor{gray!10}\textit{0.4152} & \cellcolor{gray!10}\textit{0.0290} & \cellcolor{gray!10}\textit{\textbf{0.0062}} \\
Kenansville & 0.5388 & 0.1705 & 0.2433 & 0.0476 & 0.1603 & \cellcolor{gray!10}\textit{0.4558} & \cellcolor{gray!10}\textit{0.0352} & \cellcolor{gray!10}\textit{0.0124} \\
AdvDDoS & 0.9421 & 0.3202 & 0.2650 & 0.0786 & \textbf{0.4364} & \cellcolor{gray!10}\textit{0.4672} & \cellcolor{gray!10}\textit{0.0217} & \cellcolor{gray!10}\textit{0.0093} \\
Ours & \textbf{0.9886} & \textbf{0.4012} & \textbf{0.4596} & \textbf{0.1065} & 0.3123 & \cellcolor{gray!10}\textit{\textbf{0.6712}} & \cellcolor{gray!10}\textit{\textbf{0.0373}} & \cellcolor{gray!10}\textit{0.0114} \\
\bottomrule
\end{tabular}
\end{table*}
